CABINET: Content Relevance based Noise Reduction for Table Question Answering

Table understanding capability of Large Language Models (LLMs) has been extensively studied through the task of question-answering (QA) over tables. Typically, only a small part of the whole table is relevant to derive the answer for a given question. The irrelevant parts act as noise and are distracting information, resulting in sub-optimal performance due to the vulnerability of LLMs to noise. To mitigate this, we propose CABINET (Content RelevAnce-Based NoIse ReductioN for TablE QuesTion-Answering) - a framework to enable LLMs to focus on relevant tabular data by suppressing extraneous information. CABINET comprises an Unsupervised Relevance Scorer (URS), trained differentially with the QA LLM, that weighs the table content based on its relevance to the input question before feeding it to the question-answering LLM (QA LLM). To further aid the relevance scorer, CABINET employs a weakly supervised module that generates a parsing statement describing the criteria of rows and columns relevant to the question and highlights the content of corresponding table cells. CABINET significantly outperforms various tabular LLM baselines, as well as GPT3-based in-context learning methods, is more robust to noise, maintains outperformance on tables of varying sizes, and establishes new SoTA performance on WikiTQ, FeTaQA, and WikiSQL datasets. We release our code and datasets at https://github.com/Sohanpatnaik106/CABINET_QA.

==> sections/notation.tex <==
\section{Preliminaries}

\subsection{Task Definition}
In this work, we address the task of \textit{table-based question answering}. Each instance for the underlying task consists of a table $T$, a natural language question $\mathcal{Q}$, and an answer $\mathcal{A}$. In particular, the final answer $\mathcal{A} = \{a_1, a_2, \cdots, a_n\}$ is a natural language sequence. Formally, $a_i = \text{argmax}_j P(a_j | \mathcal{Q}, T, a_1, a_2, \cdots, a_{i-1})$, where $j \in \{1, 2, \cdots, |V|\}$ and $|V|$ is the size of the vocabulary.

\subsection{Notation}
A table $T = \{c_{ij} | i < \text{Row}_T, j < \text{Col}_T \}$ contains $\text{Row}_T$ rows and $\text{Col}_T$ columns, and $c_{ij}$ represents the text present in the $i^{th}$ row and the $j^{th}$ column. Encoding the table $T$ as a sequence is non-trivial since it exhibits underlying structures. Therefore, following the scheme proposed by ~\citep{liu2022tapex}, we flatten the table into a sequence so that it can be fed directly into the model. We insert several special tokens to mention the start of column names and the rows, along with inserting a special pipe character to indicate the table boundaries. For instance, a flattened table can be represented as $\mathcal{T} = [HEAD] c_1 | c_2 | \cdots | c_{Col_T} [ROW] 1: r_1 | r_2 | \cdots r_{Row_T} [ROW] 2: \cdots $. \ys{A listing may be better for this or definitions of T, $r_1$,..} Here $[HEAD]$ and $[ROW]$ are special tokens indicating the region of table headers and rows respectively, and the number after [ROW] is used to indicate the row index. Notably, we also separate headers or cells in different columns using a pipe $|$. Finally, we prefix the flattened table $\mathcal{T}$ with the natural language query $\mathcal{Q}$ and feed them into the model.
 
\subsection{System Overview}
